Hierarchical Clustering: Objective Functions and Algorithms

Hierarchical clustering is a recursive partitioning of a dataset into clusters at an increasingly finer granularity. Motivated by the fact that most work on hierarchical clustering was based on providing algorithms, rather than optimizing a specific objective, Dasgupta framed similarity-based hierarchical clustering as a combinatorial optimization problem, where a `good' hierarchical clustering is one that minimizes some cost function. He showed that this cost function has certain desirable properties. We take an axiomatic approach to defining `good' objective functions for both similarity and dissimilarity-based hierarchical clustering. We characterize a set of "admissible" objective functions (that includes Dasgupta's one) that have the property that when the input admits a `natural' hierarchical clustering, it has an optimal value. Equipped with a suitable objective function, we analyze the performance of practical algorithms, as well as develop better algorithms. For similarity-based hierarchical clustering, Dasgupta showed that the divisive sparsest-cut approach achieves an $O(\log^{3/2} n)$-approximation. We give a refined analysis of the algorithm and show that it in fact achieves an $O(\sqrt{\log n})$-approx. (Charikar and Chatziafratis independently proved that it is a $O(\sqrt{\log n})$-approx.). This improves upon the LP-based $O(\log n)$-approx. of Roy and Pokutta. For dissimilarity-based hierarchical clustering, we show that the classic average-linkage algorithm gives a factor 2 approx., and provide a simple and better algorithm that gives a factor 3/2 approx.. Finally, we consider `beyond-worst-case' scenario through a generalisation of the stochastic block model for hierarchical clustering. We show that Dasgupta's cost function has desirable properties for these inputs and we provide a simple 1 + o(1)-approximation in this setting.

==> appx.tex <==


% \subsection{On Adversarially-Perturbed \StructInputs}

% \begin{replemma}{L:robustsimple}
%   Let $T$ be a tree output by Algorithm~\ref{alg:robustsimple},
%   let $\calN$ be the set of internal nodes of $T$.
%   For any node $N$ with children $N_1,N_2$ 
%   there exists a function $\omega: \calN \mapsto \R_+$, such that for any
%   $u \in V(N_1), v \in V(N_2)$, $\omega(N) \le w(u,v)) 
%   \le \delta \omega(N)$.
%   Moreover, for any nodes $N,N'$, if $N'$ is an ancestor of $N$,
%   we have that $\omega(N) > \omega(N')$.
% \end{replemma}


\section{Additional Proofs for Section~\ref{S:dissim:approx}}
\label{appx:dissim:approx}




  % \begin{claim}
  % Consider the output tree $T$ and the nodes $N^*_i$ corresponding
  % to the root of the subtree $T^*_{i}$.
  % We have $\forall u,v \in V(N^*_i)$, $\forall x 
  % \in V \setminus V(N^*_i)$, 
  % $\exists \omega$, such that
  % $\omega\le w(u,x)), w(v,x)) \le \delta \omega$.
  % \end{claim}
  % \begin{proof}
  %   Let $v_0$ be the first vertex in $\tilde V$.
  %   Consider the set $\tilde V$ after the
  %   creation of $B_i$, \ie $\tilde V = \bigcup_{j=1}^i B_j$.
  %   Let $u,v \in \tilde V$ such that $d(u,v)$ is maximum.
  %   By definition of an ultrametric, we have 
  %   $d(u,v_0)$ or $d(v,v_0)$ is equal to $d(u,v)$.
  %   Thus, suppose that $d(u,v_0) = d(u,v)$.
  %   For any vertex $x$ such that $d(u,x) > d(u,v) = d(u,v_0)$, 
  %   by the definition of an ultrametric, we have
  %   $\forall y \in \tilde V$, $d(y,x) \le \max(d(v_0,y),d(v_0,x)) = 
  %   d(x,v_0)$
  %   (since $d(v_0,y) \le d(u,v_0) < d(v_0,x)$).
  %   Thus, $d(y,x) = d(x,v_0)$.
  %   Hence for any point $x$, s.t. $d(u,x) > d(u,v_0)$, 
  %   since the input is a $\delta$-adversarially-perturbed
  %   graph generated from an ultrametric,
  %   we have that $\forall y \in \tilde V$, 
  %   $\delta w(x,v_0)) \ge w(x,y) \ge w(x,v_0))$.
    
  %   Let $\hat y$ be the first vertex at distance $d(u,v_0)$
  %   inserted in $\tilde V$. Let $(\hat x,\hat y)$ be the edge
  %   of maximum weight that led $\hat y$ to be inserted (and so
  %   $\hat x \in \tilde V$).
  %   If $x$ was not inserted we have that for any $y$ in
  %   $\tilde V$, $w(x,y)) < w(\hat x,\hat y))$.
  %   Now, observe that for any $y \in \tilde V$ we also have
  %   $d(y,x) \le d(v_0, \hat y) = d(\hat x,\hat y)$ and therefore,
  %   $w(\hat x,\hat y)) \ge w(y,x)) \ge w(\hat x,\hat y))/\delta $.
  % \end{proof}

  % By definition of the algorithm,
  % for any vertex $y \in B_i$, we have that 
  % $\exists s$, either $s \in B_i$ or $s \in \tvi$ and
  % $w(y,s)) = w_i$.
  % We inductively define a function $\sigma : B_i \mapsto \tvi$ 
  % as follows. For the first vertex $v^*_i$ added to $B_i$
  % we let $\sigma(v^*_i) = y$ for some $y \in \tvi$ such 
  % that $w(v^*_i,y)) = w_i$. 
  
  
  
  
%  \section{Additional Proofs for Section~\ref{S:perfectdata}}
%\label{appx:perfectdata}


%\subsection{A Faster Algorithm: 
%  Hierarchical Clustering in Near-Linear Time}
%\begin{reptheorem}{T:alg:fastsimple}
%  Algorithm~\ref{alg:fastsimple} computes a generating tree in 
%  time $O(n \log^2 n)$
%  with high probability if the input is a strongly \structinput or
%  $O(n^2)$ is the input is a \structinput.
%\end{reptheorem}

